FACTIFY-5WQA: 5W Aspect-based Fact Verification through Question Answering

Automatic fact verification has received significant attention recently. Contemporary automatic fact-checking systems focus on estimating truthfulness using numerical scores which are not human-interpretable. A human fact-checker generally follows several logical steps to verify a verisimilitude claim and conclude whether its truthful or a mere masquerade. Popular fact-checking websites follow a common structure for fact categorization such as half true, half false, false, pants on fire, etc. Therefore, it is necessary to have an aspect-based (delineating which part(s) are true and which are false) explainable system that can assist human fact-checkers in asking relevant questions related to a fact, which can then be validated separately to reach a final verdict. In this paper, we propose a 5W framework (who, what, when, where, and why) for question-answer-based fact explainability. To that end, we present a semi-automatically generated dataset called FACTIFY-5WQA, which consists of 391, 041 facts along with relevant 5W QAs - underscoring our major contribution to this paper. A semantic role labeling system has been utilized to locate 5Ws, which generates QA pairs for claims using a masked language model. Finally, we report a baseline QA system to automatically locate those answers from evidence documents, which can serve as a baseline for future research in the field. Lastly, we propose a robust fact verification system that takes paraphrased claims and automatically validates them. The dataset and the baseline model are available at https: //github.com/ankuranii/acl-5W-QA

==> img/textimg/QA_example.tex <==
\begin{tabular}{|ll|}

\hline Claim. &  \textcolor{red}{Moderna’s lawsuits against Pfizer-BioNTech show} \\ & \textcolor{red}{COVID-19 vaccines were in the works before the} \\ &  \textcolor{red}{pandemic started} \\
QA Pair1. & [( \textcolor{blue}{Who} lawsuits
against whom?, Moderna lawsuits \\ & against Pfizer-BioNTech)] \\


QA Pair2. & [( \textcolor{blue}{What} the law-
suit shows?, COVID-19 vaccines \\ & were in the works before the pandemic started. )
    ] \\

QA Pair3. & [( \textcolor{blue}{When} the
COVID-19 vaccines were in work?, \\ & before pandemic.)
    ] \\

\hline
\end{tabular}

==> img/textimg/QA_pair_evidence_example1.tex <==
\begin{tabular}{|ll|}

\hline 
\textbf{Claim:} & Moderna’s lawsuits against Pfizer-BioNTech show \\ & COVID-19 vaccines were in the works before the \\ & pandemic started.
 \\
\textbf{Evidence:} & \textcolor{blue}{Moderna is suing Pfizer and BioNTech
for patent} \\ & \textcolor{blue}{infringement}, alleging the rival companies used key \\ &  parts of its mRNA technology to develop their \\ & COVID-19 vaccine. Although the patents existed \textcolor{blue}{before} \\ & \textcolor{blue}{the pandemic began}, this does not mean Moderna or \\ & Pfizer-BioNTech were already working on the \\ & COVID-19 vaccine. 
\\
\textbf{Model Generated Question1:} & Who lawsuits against whom?, \\
\textbf{Gold Answer:} & \textcolor{orange}{Moderna lawsuits against Pfizer-BioNTech.} \\
\textbf{Answer Generated from System:} & \textcolor{blue}{Moderna} \\

\textbf{Model Generated Question2:} & What the lawsuit shows?, \\
\textbf{Gold Answer:} & \textcolor{orange}{COVID-19 vaccines were in the works before the} \\ & \textcolor{orange}{pandemic started.} \\

\textbf{Answer Generated from System:} & \textcolor{blue}{Patent infringement} \\
   
\textbf{Model Generated Question3:} & When the
COVID-19 vaccines were in work?, \\
\textbf{Gold Answer:} & \textcolor{orange}{Before pandemic.} \\

\textbf{Answer Generated from System:} & \textcolor{blue}{Before the pandemic began.} \\

\hline
\end{tabular}

% \hline Claim. &  \textcolor{red}{Moderna’s lawsuits against Pfizer-BioNTech show \\ & \textcolor{red}{COVID-19 vaccines were in the works before the} \\ &  \textcolor{red}{pandemic started}} \\
% QA Pair1. & [( \textcolor{blue}{Who} lawsuits
% against whom?, Moderna lawsuits \\ & against Pfizer-BioNTech)] \\


% QA Pair2. & [( \textcolor{blue}{What} the law-
% suit shows?, COVID-19 vaccines \\ & were in the works before the pandemic started. )
%     ] \\

% QA Pair3. & [( \textcolor{blue}{When} the
% COVID-19 vaccines were in work?, \\ & before pandemic.)
%     ] \\



==> img/textimg/srl_example.tex <==
\tiny
{
\begin{tabular}{|ll|}
\hline Claim. & \textcolor{red}{Moderna’s lawsuits against Pfizer-BioNTech}
\\ & \textcolor{red}{show COVID-19 vaccines were in} \\
& \textcolor{red}{the works before the pandemic started.} \\
\textcolor{blue}{Verbs.} & [    were, started] \\
\textcolor{blue}{Who.} & [(ARG0 : None, None)] \\
\textcolor{blue}{What.} & [(ARG1 : COVID-19 vaccines, the pandemic)] \\
\textcolor{blue}{Why.} & [(ARGM-TMP : None, None)] \\
\textcolor{blue}{When.} & [(ARGM-LOC : before the pandemic started, None) ] \\
\textcolor{blue}{Why.} & [(ARGM-TMP : None, None)] \\
\textcolor{blue}{Where.} & [(ARGM-CAU : None, None)] \\
\hline
\end{tabular}
}


==> tables/layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}
